Label Denoising through Cross-Model Agreement

Learning from corrupted labels is very common in real-world machine-learning applications. Memorizing such noisy labels could affect the learning of the model, leading to sub-optimal performances. In this work, we propose a novel framework to learn robust machine-learning models from noisy labels. Through an empirical study, we find that different models make relatively similar predictions on clean examples, while the predictions on noisy examples vary much more across different models. Motivated by this observation, we propose \em denoising with cross-model agreement \em (DeCA) which aims to minimize the KL-divergence between the true label distributions parameterized by two machine learning models while maximizing the likelihood of data observation. We employ the proposed DeCA on both the binary label scenario and the multiple label scenario. For the binary label scenario, we select implicit feedback recommendation as the downstream task and conduct experiments with four state-of-the-art recommendation models on four datasets. For the multiple-label scenario, the downstream application is image classification on two benchmark datasets. Experimental results demonstrate that the proposed methods significantly improve the model performance compared with normal training and other denoising methods on both binary and multiple-label scenarios.

==> experiments.tex <==


\section{Experiments}
In this section, we empirically demonstrate the effectiveness of the proposed DeCA(p) through enormous experiments. Specifically, two domain tasks are studied: recommendation noise and image classification noise. We aim to answer the following research questions:
\begin{itemize}[leftmargin=*]
    \item \textbf{RQ1}: How does DeCA(p) perform compared to normal training and other denoising methods? 
    \item \textbf{RQ2}: How does the design of DeCA(p) affect the recommendatin performance, namely the model selection for $h_\phi$ in Eq.(\ref{decoder})?
    \item \textbf{RQ3:} Can DeCA(p) generate reasonable preference distribution in recommendation scenario? 
\end{itemize}

\subsection{Experimental Settings}
\subsubsection{Datasets}
\begin{wraptable}{r}{8cm}
\begin{center}
\vspace{-15pt}
\caption{Statistics of the datasets}
\vspace{-10pt}
\label{tab:dataset statistics}
\resizebox{8cm}{!}{
\begin{tabular}{c|c|c|c|c}
  \toprule
  Dataset & \# Users & \# Items & \# Interactions & Sparsity \\
  \midrule
  Modcloth & 44783 & 1020 & 99893 & 0.99781 \\
%   \hline 
  Electronics & 1157633 & 9560 & 1292954 & 0.99988 \\
  \bottomrule
\end{tabular}}
\end{center}
\vspace{-0.3cm}
\end{wraptable}
We conduct comprehensive experiments on four datasets. As for recommendation tasks, we choose two public accessible datasets: Modcloth\footnote{https://modcloth.com/} and Electronics\footnote{https://github.com/MengtingWan/marketBias}. More statistics about these two datasets are shown in Table \ref{tab:dataset statistics}. We construct the clean test set with only clean examples which denote the real user preference. In terms of image classification, we use two popular datasets: CIFAR10 and Fashion-MNIST. We will add some random noise to the training set while maintaining the test set to be clean. 

\begin{itemize}[leftmargin=*]
\item \textbf{Modcloth}. It is from an e-commerce website which sells women's clothing and accessories\cite{wan2020addressing}. For evaluation, the clean test set is built on user-item pairs whose ratins scores are equal to 5\cite{wang2020denoising}. 
\item \textbf{Electronics}. Electronics is collected from the \emph{Electronics} category on Amazon \cite{ni2019justifying,wan2020addressing}.
\item \textbf{CIFAR10}. It consists of 60000 32x32 colour images in 10 classes, with 6000 images per class. There are 50000 training images and 10000 test images.
% \item \textbf{CIFAR5}. It is the dataset sampled from CIFAR10 which contains the data corresponding to the classes \{0, 1, 2, 3, 4\} in CIFAR10. 
\item \textbf{Fashion-MNIST}\cite{xiao2017/online}. It is a dataset of Zalando's article images—consisting of a training set of 60,000 examples and a test set of 10,000 examples. Each example is a 28x28 grayscale image, associated with a label from 10 classes. 
\end{itemize}

Note that all the ratings and dwell time are only used for constructing the clean test set. The recommendation model are trained only with the corrupted binary implicit feedback. 

\subsubsection{Baselines}. We select four state-of-the-art recommendation models as the target model for recommendation: 
\begin{itemize}[leftmargin=*]
    \item \textbf{GMF}~\cite{he2017neural}: This is a generalized version of MF by changing the inner product to the element-wise product and a dense layer. 
    \item \textbf{NeuMF}~\cite{he2017neural}: The method is a state-of-the-art neural CF model which combines GMF with a Multi-Layer Perceptron (MLP).
    \item \textbf{CDAE}~\cite{wu2016collaborative}: CDAE corrupts the observed interactions with random noises, and then employs several linear layers to reconstruct the original datasets, which will increase its anti-noise abilities. 
    \item \textbf{LightGCN}~\cite{he2020lightgcn}: LightGCN is a newly proposed graph-based recommendation model which learns user and item embeddings by linearly propagating them on the interaction graph.
\end{itemize}
Each model is trained with the following approaches: 
\begin{itemize}[leftmargin=*]
  \item \textbf{Normal}: Train the model on the noisy dataset with simple binary-cross-entropy (BCE) loss.
  \item \textbf{WBPR}~\cite{gantner2012personalized}: This is a re-sampling based denoising method, which considers the popular but uninteracted items are highly likely to be real negative ones.
  \item \textbf{T-CE}~\cite{wang2020denoising}: This is a re-weighting based denoising method, which uses the Truncated BCE to assign zero weights to large-loss examples with a dynamic threshold in each iteration.
  \item \textbf{Ensemble}: This is an ensemble-based approach, which aggregates the results from two models with different random seeds.
%   examples with high loss values 
  \item \textbf{DeCA(p)}: Our proposed method.
\end{itemize}

\noindent For image classification tasks, We choose ResNet-32~\cite{resnet} as the backbone model. Besides, we select the following denoising methods as the baselines: 
\begin{itemize}[leftmargin=*]
    \item \textbf{Normal}: Training on the noisy dataset. 
    \item \textbf{MW-Net}~\cite{shu2019meta}: It build a meta-weight-net to reweight the loss for each instance. The meta-weight-net is trained using a small set of clean data. In our implementaion, we select 1000 images in the whole dataset before adding noise to the remaining part, which is consistent with \cite{shu2019meta}. This serves as the re-weighting strategy mentioned in Section \ref{introduction}.
    \item \textbf{ITLM}~\cite{shen2019learning}: It uses the iterative trimmed loss strategy, select a certain portion of the dataset (\emph{eg.} 80\% of the dataset) with the minimal loss to construct a new subset, which will be used to train the model in next iteration. This serves as the re-sampling strategy mentioned in Sectioin \ref{introduction}. 
    \item \textbf{DeCA(p)}: Our proposed method.
\end{itemize}

The hyperparameters of the target model keep exactly the same (layer number, embedding size, hiddewn size, learning rate, etc.) for different approaches for fair comparisons. 

\subsection{Performance Comparison}
\subsubsection{Recommendation}. Table \ref{tab:Overall_performance} shows the performance comparison on Modcloth and Electronics. From the table, we can have following observations: (1) The proposed DeCA(p) can effectively improve the recommendation quality of the recommendation models. DeCA(p) achieves the best recall value over all settings except for few cases. (2) LightGCN perform similarly with GMF. This could be attributed to the bias of the datasets. From Table \ref{tab:dataset statistics} we can see that the users in these two datasets would only be connected to a small number of items while items are connect to a relatively large number of users. The imbalance of interaction graphs could affect the performance of LightGCN. 

\subsubsection{Image Classification}. Table \ref{tab:overall_performance_on_image_classification} shows the results of the DeCA(p) and the baselines with the backbone ResNet-32 on CIFAR10 and Fashion-MNIST. The noises are added randomly. From the table, we can have following observations: (1) Our proposed method DeCA(p) consistently outperform the normal training setting and other denoising methods. (2) As the noise ratio gets larger, our methods get less affected by the noise ratio, which means the performance gain gets more significant. 
\begin{table*}
\centering
\caption{Overall performance comparison on Image Classication task. The highest accuracies are in Boldface.}
\vspace{-0.3cm}
\label{tab:overall_performance_on_image_classification}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{c|ccccc}
\toprule
\textbf{CIFAR10} & 10\% & 20\% & 30\% & 40\% & 50\% \\
\midrule
Normal &89.01$\pm$0.41\% &87.44$\pm$0.85\% &86.06$\pm$0.55\% &84.15$\pm$0.47\% &81.83$\pm$0.77\% \\
MW-Net & 89.33$\pm$0.27\% &88.36$\pm$0.48\% &86.70$\pm$0.39\% &85.01$\pm$0.12\% &82.87$\pm$0.64\% \\
ITLM & 89.45$\pm$0.36\% &87.79$\pm$0.13\% &86.22$\pm$0.46\% &84.95$\pm$0.11\% &82.12$\pm$0.34\% \\
DeCA(p) & \textbf{90.32$\pm$0.18\%} &\textbf{88.78$\pm$0.20\%} &\textbf{87.07$\pm$0.19\%} &\textbf{86.62$\pm$0.26\%} &\textbf{84.32$\pm$0.32\%} \\
\bottomrule
% \toprule
% \textbf{CIFAR5} & 10\% & 20\% & 30\% & 40\% & 50\% \\
% \midrule
% Normal & 92.16$\pm$0.49\% & 90.90$\pm$0.43\% & 89.71$\pm$0.33\% & 87.73$\pm$0.85\% & 85.52$\pm$0.75\% \\
% MW-Net & 92.62$\pm$0.12\% & 91.19$\pm$0.50\% & 90.01$\pm$0.62\% & 88.11$\pm$0.60\% & 86.12$\pm$0.13\% \\
% ITLM & 92.65$\pm$0.10\% & 90.00$\pm$0.19\% & 88.91$\pm$0.55\% & 88.21$\pm$0.92\% & 85.66$\pm$0.32\% \\
% DVAE & \textbf{92.70$\pm$0.20\%} &\textbf{91.26$\pm$0.30\%} &\textbf{90.09$\pm$0.21\%} &\textbf{89.30$\pm$0.30\%} &\textbf{86.69$\pm$0.29\%} \\
% \bottomrule
\toprule
\textbf{FMNIST}& 10\% & 20\% & 30\% & 40\% & 50\% \\
\midrule
Normal & 87.01$\pm$0.02\% &86.42$\pm$0.03\% &85.58$\pm$0.02\% &84.89$\pm$0.02\% &83.62$\pm$0.02\% \\
MW-Net & 88.01$\pm$0.08\% &86.54$\pm$0.10\%&86.81$\pm$0.08\% &86.18$\pm$0.09\% &84.37$\pm$0.07\% \\
ITLM & 89.01$\pm$0.09\% &88.55$\pm$0.06\% &87.56$\pm$0.04\% &87.10$\pm$0.08\% &86.53$\pm$0.06\% \\
DeCA(p) & \textbf{89.47$\pm$0.05\%} &\textbf{89.44$\pm$0.03\%} &\textbf{88.86$\pm$0.04\%} &\textbf{88.72$\pm$0.06\%} &\textbf{88.25$\pm$0.07\%} \\
\bottomrule
\end{tabular}
% \vspace{-0.5cm}
% \vspace{-5pt}
\end{table*}

\begin{table*}
\centering
\caption{Overall performance comparison on recommendation tasks. The highest scores are in Boldface. R is short for Recall and N is short for NDCG.}
\vspace{-0.3cm}
\label{tab:Overall_performance}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc|cccc}
\toprule
\multirow{2}{*}{\textbf{Modcloth}}& R@5 & R@20 &N@5 &N@20 & R@5 & R@20 &N@5 &N@20 \\
\cmidrule(lr){2-5}\cmidrule{6-9} 
&\multicolumn{4}{c|}{GMF} & \multicolumn{4}{c}{NeuMF} \\ 
    \midrule
Normal & 0.063$\pm$0.006 & 0.225$\pm$0.008 & 0.043$\pm$0.005 & 0.088$\pm$0.005 & 0.082$\pm$0.003 & 0.242$\pm$0.004 & 0.055$\pm$0.002 & 0.101$\pm$0.002 \\
WBPR & 0.067$\pm$0.002 & 0.224$\pm$0.002 & 0.046$\pm$0.001 & 0.090$\pm$0.001 & \textbf{0.092$\pm$0.001} & 0.247$\pm$0.020 & \textbf{0.064$\pm$0.001} & 0.108$\pm$0.006 \\
T-CE & 0.067$\pm$0.004 & 0.235$\pm$0.002 & 0.045$\pm$0.003 & 0.093$\pm$0.001 & 0.065$\pm$0.010 & 0.228$\pm$0.008 & 0.044$\pm$0.010 & 0.091$\pm$0.008 \\
Ensemble & 0.064$\pm$0.004 & 0.228$\pm$0.007 & 0.043$\pm$0.002 & 0.089$\pm$0.002 & 0.090$\pm$0.003 & 0.260$\pm$0.004 & 0.061$\pm$0.001 & 0.109$\pm$0.002 \\ 
DeCA(p) & \textbf{0.074$\pm$0.001$^*$} & \textbf{0.247$\pm$0.001$^*$} & \textbf{0.052$\pm$0.001$^*$} & \textbf{0.100$\pm$0.000$^*$} & 0.087$\pm$0.005 & \textbf{0.265$\pm$0.006} & 0.059$\pm$0.004 & \textbf{0.110$\pm$0.004} \\
\hline
& \multicolumn{4}{c|}{CDAE} & \multicolumn{4}{c}{LightGCN} \\ 
\hline
Normal & 0.082$\pm$0.004 & 0.242$\pm$0.003 & 0.052$\pm$0.002 & 0.098$\pm$0.001 & 0.065$\pm$0.001 & 0.220$\pm$0.002 & 0.043$\pm$0.001 & 0.087$\pm$0.002 \\
WBPR & 0.079$\pm$0.000 & 0.238$\pm$0.004 & 0.050$\pm$0.000 & 0.095$\pm$0.001 & 0.072$\pm$0.001 & 0.222$\pm$0.002 & 0.046$\pm$0.001 & 0.088$\pm$0.001 \\
T-CE & 0.075$\pm$0.003 & 0.243$\pm$0.008 & 0.048$\pm$0.002 & 0.096$\pm$0.002 & 0.071$\pm$0.000 & 0.231$\pm$0.001 & 0.049$\pm$0.000 & 0.093$\pm$0.000 \\
Ensemble & 0.084$\pm$0.002 & 0.250$\pm$0.002 & 0.054$\pm$0.001 & 0.100$\pm$0.001 & 0.068$\pm$0.001 & 0.227$\pm$0.001 & 0.046$\pm$0.000 & 0.090$\pm$0.000 \\ 
DeCA(p) & \textbf{0.089$\pm$0.004$^*$} & \textbf{0.251}$\pm$0.005 & \textbf{0.057$\pm$0.003$^*$} & \textbf{0.103$\pm$0.003$^*$} & \textbf{0.073$\pm$0.001} & \textbf{0.235$\pm$0.001} & \textbf{0.051$\pm$0.001} & \textbf{0.096$\pm$0.000} \\
\bottomrule
\toprule
 \multirow{2}{*}{\textbf{Electronics}} & R@10 & R@50 &N@10 &N@50 & R@10 & R@50 &N@10 &N@50 \\
\cmidrule(lr){2-5}\cmidrule{6-9} 
 & \multicolumn{4}{c|}{GMF} & \multicolumn{4}{c}{NeuMF} \\ 
    \hline
Normal & 0.023$\pm$0.000 & 0.063$\pm$0.001 & 0.013$\pm$0.000 & 0.021$\pm$0.000 & 0.075$\pm$0.000 & 0.191$\pm$0.002 & 0.048$\pm$0.000 & 0.072$\pm$0.001 \\
WBPR & 0.026$\pm$0.001 & 0.072$\pm$0.001 & 0.014$\pm$0.000 & 0.024$\pm$0.000 & \textbf{0.077}$\pm$0.000 & \textbf{0.201}$\pm$0.001 & \textbf{0.048}$\pm$0.000 & 0.074$\pm$0.000 \\
T-CE & 0.024$\pm$0.000 & 0.063$\pm$0.001 & 0.013$\pm$0.000 & 0.022$\pm$0.000 & 0.071$\pm$0.004 & 0.189$\pm$0.008 & 0.045$\pm$0.002 & 0.071$\pm$0.003 \\
Ensemble & 0.014$\pm$0.001 & 0.034$\pm$0.001 & 0.010$\pm$0.000 & 0.016$\pm$0.000 &  0.051$\pm$0.000 & 0.108$\pm$0.001 & 0.040$\pm$0.000 & 0.055$\pm$0.000 \\
DeCA & \textbf{0.045$\pm$0.001$^*$} & 0.104$\pm$0.000 & 0.023$\pm$0.000 & 0.037$\pm$0.000 & 0.071$\pm$0.001 & 0.191$\pm$0.001 & 0.044$\pm$0.002 & 0.069$\pm$0.001 \\
DeCA(p) & 0.042$\pm$0.001 & \textbf{0.110$\pm$0.000$^*$} & \textbf{0.024$\pm$0.000$^*$} & \textbf{0.038$\pm$0.000$^*$} & 0.074$\pm$0.002 & 0.200$\pm$0.001 & 0.047$\pm$0.000 & \textbf{0.074}$\pm$0.000 \\
\hline
& \multicolumn{4}{c|}{CDAE} & \multicolumn{4}{c}{LightGCN} \\ 
\hline
Normal & 0.074$\pm$0.001 & 0.197$\pm$0.001 & 0.047$\pm$0.000 & 0.073$\pm$0.000 & 0.024$\pm$0.000 & 0.081$\pm$0.001 & 0.016$\pm$0.000 & 0.030$\pm$0.000 \\
WBPR & 0.077$\pm$0.000 & 0.190$\pm$0.000 & 0.048$\pm$0.000 & 0.072$\pm$0.000 & 0.022$\pm$0.000 & 0.076$\pm$0.001 & 0.015$\pm$0.000 & 0.028$\pm$0.000 \\
T-CE & 0.067$\pm$0.002 & 0.187$\pm$0.010 & 0.044$\pm$0.001 & 0.067$\pm$0.003 & 0.024$\pm$0.001 & 0.086$\pm$0.001 & 0.017$\pm$0.000 & 0.031$\pm$0.000 \\
Ensemble & 0.043$\pm$0.000 & 0.110$\pm$0.001 & 0.036$\pm$0.000 & 0.056$\pm$0.000 & 0.018$\pm$0.000 & 0.049$\pm$0.001 & 0.014$\pm$0.000 & 0.023$\pm$0.000 \\
DeCA(p) & \textbf{0.077$\pm$0.000} & \textbf{0.202}$\pm$0.001 & \textbf{0.048}$\pm$0.000 & \textbf{0.075}$\pm$0.000 & \textbf{0.026}$\pm$0.001 & \textbf{0.104$\pm$0.001$^*$} & \textbf{0.019}$\pm$0.000 & \textbf{0.037$\pm$0.000$^*$} \\
\bottomrule
\end{tabular}}
\vspace{-0.5cm}
% \vspace{-5pt}
\end{table*}


To conclude, the proposed DeCA(p) achieves consistent and significant improvements compared with other methods, which demonstrates the effectiveness and generalization ability of our methods.



\subsection{Model Investigation}
\subsubsection{Training Curve}
\begin{wrapfigure}{r}{0.6\textwidth}
\vspace{-0.8cm}
\centering     %%% not \center
\subfigure[GMF on Modcloth]{\label{fig:GMF_modcloth_recall}\includegraphics[width=0.49 \linewidth]{figures/GMF_modcloth.pdf}}
\subfigure[ResNet on CIFAR10]{\label{fig:CIFAR10_acc}\includegraphics[width=0.47 \linewidth]{figures/CIFAR10.pdf}}
% \includegraphics[width=\linewidth]{figures/GMF_modcloth.png}
% \subfigure[Adressa]{\label{fig:GMF_adressa_recall}\includegraphics[width=0.494\linewidth]{pictures/GMF_adressa_recall.png}}
\vspace{-0.6cm}
\caption{Model performance along the training process.}
\vspace{-0.5cm}
\label{fig:Analysis_on_memorizing_noisy_samples}
\end{wrapfigure}
We have analysised how DeCA(p) affect the memorization of noisy samples, i.e. enhance the robustness of the mdoel. Figure shows the learning curve of normal training and the proposed DeCA(p) with GMF on Modcloth for recommendation, and with ResNet32 on CIFAR10 for image classification. From the results, we could find that the problem of memorizing noisy samples is severe in normal training and also in other denoising methods. However, for DeCA(p), the performance remain stable and better along the whole training stage. The results demonstrate that the proposed DeCA(p) successfully prevent the model from being affected by noisy samples. Besides, even though the other methods may achieve the accuracy that is compatible to ours, the validation set may still fail to help choose the checkpoint with the highest accuracy. Thus our method DeCA(p) is still needed. 


\subsubsection{Hyperparameter Sensitivity}
\begin{wrapfigure}{r}{0.6\textwidth}
\vspace{-0.8cm}
\centering     %%% not \center
\subfigure[GMF on Modcloth]{\label{fig:GMF_modcloth_hyper}\includegraphics[width=0.49 \linewidth]{figures/GMF_modcloth_DVAE.png}}
\subfigure[ResNet on CIFAR10]{\label{fig:CIFAR10_hyper}\includegraphics[width=0.49 \linewidth]{figures/CIFAR10_hyper.png}}
% \includegraphics[width=\linewidth]{figures/GMF_modcloth.png}
% \subfigure[Adressa]{\label{fig:GMF_adressa_recall}\includegraphics[width=0.494\linewidth]{pictures/GMF_adressa_recall.png}}
\vspace{-0.6cm}
\caption{Hyperparameter Sensitivity}
\vspace{-0.8cm}
\label{fig:Hyperparameter_sensitivity}
\end{wrapfigure}
DeCA(p) contain two hyperparameters $C_1$ and $C_2$ in the early iterative training routine. A larger $C_1$ means we are more confident that the examples of current class are more likely to be clean, while a larger $C_2$ generally means we tend to believe that the examples from classes other than the current class are clean.  


\subsubsection{Model Interpretation}
\begin{wrapfigure}{r}{0.6\textwidth}
\vspace{-0.2cm}
\centering     %%% not \center
\subfigure[Modcloth]{\label{fig:modcloth_ratings_DPI}\includegraphics[width=0.493\linewidth]{figures/modcloth_ratings_DVAE.pdf}}
\subfigure[Electronics]{\label{fig:modcloth_ratings_DVAE}\includegraphics[width=0.493\linewidth]{figures/electronics_5_ratings_DVAE.pdf}}
\vspace{-0.3cm}
\caption{Mean real positive probability of different ratings on Modcloth. Model names in the legend denote different $h$ and $h'$.}
\vspace{-0.5cm}
\label{fig:modcloth_ratings}
\end{wrapfigure}
In this part, we conduct experiments to see whether DeCA(p) generate the reasonable user preference distribution given the corrupted data observation. The real positive probability (i.e., $P(r_{ui}=1|\tilde{r}_{ui}=1)$) describes the probability of an interacted sample to be real positive. 
For DeCA(p), $P(r_{ui}=1|\tilde{r}_{ui}=1)$ can be directly computed as $P(r_{ui}=1|\tilde{r}_{ui}=1)= f_\theta(u, i)$ with condition $\tilde{r}_{ui}=1$.
Figure \ref{fig:modcloth_ratings} shows the relationship between ratings and the mean real positive probability (i.e., $P(r_{ui}=1|\tilde{r}_{ui}=1)$) on Modcloth. Results on Electronics are shown in the supplement.
We can see that the probability gets larger as the ratings go higher, which is consistent with the  impression that examples with higher ratings should be more likely to be real positive. 
%indicate that our methods are capable of detecting noisy samples, thus to avoid the model to be affected by these noisy samples. 
Besides, we can see that the probability trend is consistent with different $h$ and $h'$ models, which further demonstrate the generalization ability of our methods.






% \begin{table}
%     \centering
%     \caption{Overall Performance with ResNet32 on the first 5-class of CIFAR10 with Random Label Error}
%     \vspace{-8pt}
%      \label{tab:overall_performance_random}
%     \begin{tabular}{ccccc}
%     \hline
%         Noise Rate & Normal & MW-net & ITLM & DVAE  \\
%         \hline
%         \hline
%         10\% & 92.16$\pm$0.49\% & 92.62$\pm$0.12\% & 92.65$\pm$0.10\% & \textbf{92.70$\pm$0.20\%} \\
%         20\% & 90.90$\pm$0.43\% & 91.19$\pm$0.50\% & 90.00$\pm$0.19\% & \textbf{91.26$\pm$0.30\%} \\
%         30\% & 89.71$\pm$0.33\% & 90.01$\pm$0.62\% & 88.91$\pm$0.55\%  & \textbf{90.09$\pm$0.21\%} \\
%         40\% & 87.73$\pm$0.85\% & 88.11$\pm$0.60\% & 88.21$\pm$0.92\%  & \textbf{89.30$\pm$0.30\%} \\
%         50\% & 85.52$\pm$0.75\% & 86.12$\pm$0.13\% & 85.66$\pm$0.32\% & \textbf{86.69$\pm$0.29\%} \\
%         \hline
%     \end{tabular}
% \end{table}



% \begin{table}
%     \centering
%     \caption{Overall Performance on 10\% sub-sampled Fashion-MNIST with Random Label Error}
%     \vspace{-8pt}
%     \label{tab:overall_performance_random}
%     \begin{tabular}{ccccc}
%     \hline
%         Noise Rate & Normal & MW-net & ITLM & DVAE  \\
%         \hline
%         \hline
%         10\% & 79.54$\pm$0.02\% & & & 84.66$\pm$0.03\% \\
%         20\% & 78.76$\pm$0.03\% & & & 84.14$\pm$0.04\%\\
%         30\% & 77.40$\pm$0.02\% & & & 83.52$\pm$0.06\% \\
%         40\% & 76.53$\pm$0.03\% & & & 83.12$\pm$0.05\% \\
%         50\% & 74.18$\pm$0.02\% & & & 81.66$\pm$0.04\% \\
%         \hline
%     \end{tabular}
% \end{table}

==> method.tex <==
\section{METHODOLOGY} % (fold)
\label{sec:method}
In this section, we propose the learning framework DeCA which uses the observations described in section \ref{sec:motivation} as the denoising signals to learn robust machine learning models. We first describe the denoising for binary implicit feedback recommendation, then we generalize the method for multi-class image classification.
\subsection{Denoising for Implicit Feedback Recommendation}
Before the detailed description of the methods,  we first present some notations and problem formulation.
\subsubsection{Notations and Problem Formulation}
\label{sub:notations_and_problem_formulation}
%In this section, we first give some notations in our work. Then we will describe our methods in detail.
% Then we will briefly describe the basic routine in recommender system training and demonstrate the binary cross-entropy loss in a probabilistic way so that it can be unified with our methods later. 
We use $u\in\mathcal{U}$ and $i\in \mathcal{I}$ to denote the user and item with $\mathcal{U}$ and $\mathcal{I}$ being the user and item sets respectively.
$\tilde{\textbf{R}} \in \mathbb{R}^{|\mathcal{U}|\times |\mathcal{I}|}$ is the binary matrix for corrupted data. $\tilde{r}_{ui}$ represents the $(u,i)$-th entry of $\tilde{\textbf{R}}$ and is defined as $\tilde{r}_{ui}=1$ if there is an 
% observed interaction %%%
interaction
between user $u$ and item $i$, otherwise $\tilde{r}_{ui}=0$. Due to the existence of noisy examples, the real preference matrix is different from $\tilde{\textbf{R}}$. We use $\textbf{R}\in \mathbb{R}^{|\mathcal{U}|\times |\mathcal{I}|}$ to denote the real preference matrix and $r_{ui}$ is the real preference of user $u$ over item $i$. What we have is the corrupted binary $\tilde{\textbf{R}}$ while the clean $\textbf{R}$ is not accessible.

Formally, we assume $r_{ui}$ is drawn from a Bernoulli distribution:
\begin{equation}
\label{rui-berno}
  r_{ui} \sim Bernoulli(\eta_{ui})\approx Bernoulli(f_\theta(u,i)),
\end{equation} 
where $\eta_{ui}$ describes the probability of positive preference (i.e., $r_{ui}=1$) and is approximated by $f_\theta(u,i)$. $\theta$ denotes the parameters of $f$. We use $f_\theta$ as our target recommender that generates the final recommendation. Specifically, the output value after sigmoid of the logits from the model is denoted as $f_\theta(u, i)$, which is also the probability that $\eta_{ui}$ equals to 1. Generally speaking, $f_\theta$ is expected to have high model expressiveness. Since the denoising signal comes from the agreement across different model predictions, we introduce another auxiliary Bernoulli distribution parameterized by $g_\mu(u,i)$,  In this paper, we use a relatively simple model matrix factorization (MF) \cite{koren2009matrix} as the auxiliary model $g_\mu$. Recent research has demonstrated that MF is still one of the most effective models to capture user preference for recommendation \cite{rendle2020neural}. 

Considering both the noisy positive and noisy negative examples, we assume that given the real preference $r_{ui}$, the corrupted binary $\tilde{r}_{ui}$ is also drawn from Bernoulli distributions as
\begin{equation}\label{h_model}
  \begin{array}{c}
  \tilde{r}_{ui}|r_{ui}=0 \sim Bernoulli(h_\phi(u,i))\\
  \tilde{r}_{ui}|r_{ui}=1 \sim Bernoulli(h'_\psi(u,i)),
  \end{array}
\end{equation}
where $h_\phi(u,i)$ and $h'_\psi(u,i)$, parameterized by $\phi$ and $\psi$ respectively, are two models describing the consistency between the real user preference and data observation. We use two MF models as $h$ and $h'$ without special mention.

The task of this paper is, %\textcolor{red}{Our task/aim is}: 
given the corrupted binary data $\tilde{\textbf{R}}$, to infer the real user preference $\textbf{R}$ and its underlying model $f_\theta$, then to use $f_\theta$ to generate recommendation.

\subsubsection{Denoising with Cross-Model Agreement} % (fold)
\label{sub:denoising_with_variational_inference}
As discussed in section \ref{sec:motivation}, for clean examples which denote the real user preference, different models tend to make more consistent predictions compared with noisy examples. 
For simplicity, in this subsection we use $P(\mathbf{R})$ to denote the real user preference $Bernoulli(\eta)$. $P_f(\textbf{R})$ and $P_g(\textbf{R})$ are used to represent the approximated $Bernoulli(f_\theta)$ and $Bernoulli(g_\mu)$, correspondingly.

Due to the fact that $P_f(\textbf{R})$ and $P_g(\textbf{R})$ both approximate the real user preference $\textbf{R}$, they should remain a relatively small KL-divergence according to section \ref{sec:motivation}, which is formulated as 
\begin{equation}
\label{eq:kl-original}
D[P_g(\textbf{R})||P_f(\textbf{R})]=E_{\textbf{R}\sim P_g}[\log P_g(\textbf{R})-\log P_f(\textbf{R})].
\end{equation}
However, naively optimizing Eq.(\ref{eq:kl-original}) is meaningless since we do not have the supervision signal of $\mathbf{R}$. As a result, we need to introduce supervision signals from the corrupted data observation $\tilde{\textbf{R}}$. Using the Bayes theorem, $P_f(\textbf{R})$ can be approximated as 
\begin{equation}
\label{eq:bayesian}
P_f(\textbf{R})\approx P(\textbf{R})=\frac{P(\tilde{\textbf{R}}) P(\textbf{R}|\tilde{\textbf{R}})}{P(\tilde{\textbf{R}}|\textbf{R})}.
\end{equation}
Combining Eq.(\ref{eq:bayesian}) and Eq.(\ref{eq:kl-original}), we can obtain
\begin{align}
\label{eq:transformation}
   D&[P_g(\textbf{R}) || P_f(\textbf{R})] = E_{\textbf{R} \sim P_g}[\log P_g(\textbf{R}) - \log P_f(\textbf{R})] \nonumber \\
  &\approx E_{\textbf{R} \sim P_g} [\log P_g(\textbf{R}) - \log \frac{P(\tilde{\textbf{R}}) P(\textbf{R}|\tilde{\textbf{R}})}{P(\tilde{\textbf{R}}|\textbf{R})}] \nonumber \\
  &= E_{\textbf{R} \sim P_g}[\log P_g(\textbf{R}) - \log P(\textbf{R}|\tilde{\textbf{R}}) - \log P(\tilde{\textbf{R}}) + \log P(\tilde{\textbf{R}}|\textbf{R})]  \nonumber \\
  &= D[P_g(\textbf{R})||P(\textbf{R}|\tilde{\textbf{R}})] - \log P(\tilde{\textbf{R}}) + E_{\textbf{R} \sim P_g}[\log P(\tilde{\textbf{R}}|\textbf{R})].
\end{align}
We then rearrange the terms in Eq.(\ref{eq:transformation}) and obtain
\begin{align}
  E_{\textbf{R} \sim P_g}[\log P(\tilde{\textbf{R}}|\textbf{R})] &- D[P_g(\textbf{R}) || P_f(\textbf{R})] \nonumber \\
  &= \log P(\tilde{\textbf{R}}) - D[P_g(\textbf{R})||P(\textbf{R}|\tilde{\textbf{R}})]. \label{lower_bound}
\end{align}
We can see the meaning of maximizing the left side of Eq.(\ref{lower_bound}) is maximizing the likelihood of data observation given real user preference (i.e., $\log P(\tilde{\textbf{R}}|\textbf{R})$) and meanwhile minimizing the KL-divergence between two models which both approximate the real user preference (i.e., $D[P_g(\textbf{R}) || P_f(\textbf{R})]$).
Since the KL-divergence $D[P_g(\textbf{R})||P(\textbf{R}|\tilde{\textbf{R}})]$ is larger than zero, the left side of Eq.(\ref{lower_bound}) can also be seen as the lower bound of $\log P(\tilde{\textbf{R}})$. The bound is satisfied only if $P_g(\textbf{R})$ perfectly recovers $P(\textbf{R}|\tilde{\textbf{R}})$, in other words, $P_g(\textbf{R})$ perfectly approximates the real user preference given the corrupted data.

A naive solution is to directly maximize the left side of Eq.(\ref{lower_bound}) with an end-to-end fashion. However, it would not yield satisfactory performance. The reason is that the left side of Eq.(\ref{lower_bound}) is based on the expectation over $P_g$. The learning process is equivalent to training $g_\mu$ with the corrupted data $\tilde{\textbf{R}}$ and then uses $D[P_g(\textbf{R})||P_f(\textbf{R})]$ to transmit the information from $g_\mu$ to $f_\theta$. However, the information is 
corrupted 
and it will affect the performance of our target model $f_\theta$. To fix the problem, we notice that when the training process is converged, two distributions $P_f(\textbf{R})$ and $P_g(\textbf{R})$ would be close to each other.
We can then modify the left side of Eq.(\ref{lower_bound})
as
\begin{align}
  \label{trick}
  E_{\textbf{R} \sim P_f}[\log P(\tilde{\textbf{R}}|&\textbf{R})] - D[P_g(\textbf{R}) || P_f(\textbf{R})] \nonumber \\
  &\approx \log P(\tilde{\textbf{R}}) - D[P_g(\textbf{R})||P(\textbf{R}|\tilde{\textbf{R}})].
\end{align}


Then optimizing the left side of Eq.(\ref{trick}) is actually training $f_\theta$ with the corrupted $\tilde{\textbf{R}}$ and then transmit information to $g_\mu$. However, since $g_\mu$ is relatively simple than $f_\theta$, $g_\mu$ could only fit the robust data component (i.e., clean examples). 
Thus $g_\mu$ would not affect the learning of $f_\theta$ on clean examples, while in the meantime, pull back $f_\theta$ on noisy samples, or in other words, 
% Then $g_\mu$ will in turn help $f_\theta$ to enhance the learning on clean examples while
downgrade the noisy signal. To this end, the denoising objective function can be formulated as
\begin{align}
  \label{L_simple}
  \mathcal{L}=-E_{\textbf{R} \sim P_f}[\log P(\tilde{\textbf{R}}|\textbf{R})]+D[P_g(\textbf{R}) || P_f(\textbf{R})].
\end{align}
Considering that the gradient of $D[P_g||P_f]$ and $D[P_f||P_g]$ to $\theta$ is different, which could slightly affect the performance, we then formulate the final denoising objective function as
\begin{equation}
  \mathcal{L}_{DeCA} = -E_{\textbf{R}\sim P_f}[\log P(\tilde{\textbf{R}}|\textbf{R})] + \alpha D[P_g||P_f] + (1-\alpha)D[P_f||P_g],
  \label{DPI-loss}
\end{equation}
where $\alpha \in [0,1]$ is a hyper-parameter.


In fact, the two models $f_\theta$ and $g_\mu$ in Eq.(\ref{DPI-loss}) can play a symmetric role, but we still need a model (here we use $f_\theta$) to do the inference. Thus, the other model (here we use $g_\mu$) serves as an auxiliary model. For Co-trained DeCA, we chose $g_\mu$ to be MF to (1)  achieve more efficient computation and more stable learning because of the simplicity of MF; (b) yield good performances since MF is shown to be still effective (as stated in Section \ref{sub:notations_and_problem_formulation}); (c) make the proposed DeCA more applicable without tuning on the selection of $g_\mu$, as MF is one of the most general models. 
% More precisely, we can give the detailed formulation of the terms of \ref{DPI-loss} in Supplement \ref{ssub:mathematical_formulation}.  



\subsubsection{DeCA with Fixed Pre-training}
As described in subsection \ref{sub:denoising_with_variational_inference}, DeCA utilizes an auxiliary model $g_\mu$ as an information filter which helps to downgrade the effect of noisy signal. The auxiliary model $g_\mu$ is co-trained jointly with the target model $f_\theta$. As discussed before, the left side of Eq.(\ref{lower_bound}) is the lower bound of $\log P(\tilde{\textbf{R}})$, which is satisfied when $P_g(\mathbf{R}) \approx P(\textbf{R}|\tilde{\textbf{R}})$. Then as the training process converge, we have $P_g(\mathbf{R}) \approx P_f(\mathbf{R}) $. Thus we could expect $P(\textbf{R}|\tilde{\textbf{R}}) \approx P_f(\mathbf{R})$.


To this end, we modify the assumption of Eq.(\ref{rui-berno}) as 
\begin{equation}
\label{rui|r-berno}
  r_{ui}|\tilde{r}_{ui} \sim Bernoulli(\eta_{ui})\approx Bernoulli(f_\theta(u,i)).
\end{equation} 
The underlying intuition is that whether the data observation is known or not should not affect the robust real user preference, which is reasonable and keeps inline with the nature of robust learning. 
As a result, we should minimize the following KL-divergence
\begin{equation}
    D[P_f(\textbf{R}|\tilde{\textbf{R}}) || P(\textbf{R}|\tilde{\textbf{R}})].
\end{equation}
Through Bayesian transformation, the following equation can be deduced:
\begin{equation}
\label{VAE_lower_bound}
E_{P_f}[\log P(\tilde{\textbf{R}}|\textbf{R})] - D[P_f(\textbf{R}|\tilde{\textbf{R}})|| P(\textbf{R})] \nonumber = \log P(\tilde{\textbf{R}}) - D[P_f(\textbf{R}|\tilde{\textbf{R}})||P(\textbf{R}|\tilde{\textbf{R}})].
\end{equation}
Similarly with Eq.(\ref{DPI-loss}), we propose another variant loss function as DeCA with pre-training (DeCA(p)): 
\begin{align}
\label{DVAE-loss}
  \mathcal{L}_{DeCA(p)} &= - E_{P_f}[\log P(\tilde{\textbf{R}}|\textbf{R})] + \alpha D[P_f(\textbf{R}|\tilde{\textbf{R}}) || P(\textbf{R})] + (1- \alpha)D[P(\textbf{R}) || P_f(\textbf{R}|\tilde{\textbf{R}})].
\end{align}

The detailed formulation of the term $E_{\textbf{R}\sim P_f}[\log P(\tilde{\textbf{R}}|\textbf{R})]$ in $\mathcal{L}_{DeCA}$ is shown as: 
\begin{align}
\small
  &E_{\textbf{R}\sim P_f}[\log P(\tilde{\textbf{R}}|\textbf{R})] = \sum_{(u,i)} E_{r_{ui}\sim P_f} [\log P(\tilde{r}_{ui}|r_{ui})] \nonumber \\
  &=\sum_{(u,i)|\tilde{r}_{ui}=1}  \left\{\begin{array}{ll}
    \log P(\tilde{r}_{ui}=1|r_{ui}=1) \cdot P_f(r_{ui}=1) \\+
     \log P(\tilde{r}_{ui}=1|r_{ui}=0)\cdot P_f(r_{ui}=0) \end{array}\right. \nonumber\\
     &+\sum_{(u,i)|\tilde{r}_{ui}=0} \left\{\begin{array}{ll}
    \log P(\tilde{r}_{ui}=0|r_{ui}=1) \cdot P_f(r_{ui}=1) \\
    + \log P(\tilde{r}_{ui}=0|r_{ui}=0)\cdot P_f(r_{ui}=0)
  \end{array}\right. \nonumber \\
  &=\hspace{-0.3cm}\sum_{(u,i)|\tilde{r}_{ui}=1}\hspace{-0.3cm}
    \log h'_\psi(u,i) \cdot f_{\theta}(u,i) + \log h_\phi(u,i) \cdot (1-f_\theta(u,i))\nonumber \\
  &+\hspace{-0.3cm}\sum_{(u,i)|\tilde{r}_{ui}=0}\hspace{-0.3cm}
  \log(1 - h'_\psi(u,i))\cdot f_{\theta}(u,i) + \log(1 - h_\phi(u,i) ) \cdot (1-f_\theta(u,i)).
  \label{eq:likelihood}
\end{align}
The KL divergence term $D[P_g||P_f]$ can be calculated as
\begin{equation*}
  D[P_g||P_f] = g_\mu(u,i) \cdot \log \frac{g_\mu(u,i)}{f_\theta(u,i)} + (1-g_\mu(u,i)) \cdot \log \frac{1 - g_\mu(u,i)}{1-f_\theta(u,i)}.
\end{equation*}
$D[P_f||P_g]$ is computed similarly with $D[P_g||P_f]$.

We use a pre-trained model $f_{\theta'}$ which has the same structure as our target model $f_\theta$ but is trained with different random seeds to model $P(\mathbf{R})$. This setting is motivated by the observation that one model trained with different random seeds tends to make high variance predictions on noisy examples but more consistent agreement predictions on clean examples, as shown in Figure \ref{fig:Different_random_seeds}. 

The major difference between DeCA and DeCA(p) can be summarized as follows:
\begin{itemize}[leftmargin=*]
  \item The auxiliary model $g_\mu$ of DeCA is a simple MF while the involved $f_{\theta'}$ in DeCA(p) has the same structure as the target model.
  \item DeCA co-trains the auxiliary model $g_\mu$ with $f_\theta$ but DeCA(p) uses a pre-trained and fixed $f_{\theta'}$ to describe the prior distribution.
\end{itemize}


\subsubsection{Training Routine} % (fold)
\label{sub:training_routine}
We can see that the objective functions of both DeCA and DeCA(p) contain the term of $E[\log P(\tilde{\textbf{R}}|\textbf{R})]$.
A naive solution to optimize $E[\log P(\tilde{\textbf{R}}|\textbf{R})]$ is direct performing calculation as shown in Eq.(\ref{eq:likelihood}).
However, we find that it won't yield satisfactory results. 
The reason is that computing $E[\log P(\tilde{\textbf{R}}|\textbf{R})]$ involves updating three models $h_\phi$, $h'_\psi$ and $f_\theta$ simultaneously. Then these models will interfere with each other. The corrupted outputs from $h_\phi$ and $h'_\psi$ will prevent $f_\theta$ from learning well, and vice versa. 
To handle this issue, we split the denoising problem into two dual tasks: \emph{Denoising Positive} (DP) which aims to denoise the noisy positive examples from interacted samples. 
% as shown in Figure \ref{fig:FN}; 
and \emph{Denoising Negative} (DN) which aims to denoise noisy negative examples from sampled missing interactions.
% as illustrated in Figure \ref{fig:FP}. 
We then optimize these two sub-tasks iteratively. 
% \wy{Each time we only consider either $h_\phi$ or $h'_\psi$, and fix the other one to be the function of an approximate large value denoted as $C_1$ and $C_2$ as illustrated in the following part. Then we can obtain information from the data to update $f_\theta$, and also refine one of the $h$-models according to the outputs of $f_\theta$.}
 
\textbf{Denoising Positive}. % (fold)
In this situation, we only focus on denoising  noisy positive examples, which means we will regard every negative sample as a clean example. That is to say,
given $r_{ui} = 1$ we will always have $\tilde{r}_{ui}=1$ (i.e., $h'_\psi(u,i)=1$). %Thus we don't need to care about the distribution $\tilde{r}_{ui}|r_{ui}=1$ in \ref{h_model}, or we freeze $h_\psi'(u,i)$ to be 1. 
Thus in this sub-task, only the model $h_\phi$ will be trained.
Then the term $E[\log P(\tilde{\textbf{R}}|\textbf{R})]$ becomes
\begin{align}
\label{eq:likelihood-dfp}
  &E[\log P(\tilde{\textbf{R}}|\textbf{R})]=\hspace{-0.3cm}\sum_{(u,i)|\tilde{r}_{ui}=1}\hspace{-0.3cm}
     \log h_\phi(u,i) \cdot (1-f_\theta(u,i))\nonumber \\
   &-\hspace{-0.3cm}\sum_{(u,i)|\tilde{r}_{ui}=0}\hspace{-0.3cm}
  C_1\cdot f_{\theta}(u,i) + \log(1 - h_\phi(u,i) ) \cdot (1-f_\theta(u,i)),
\end{align}
where $C_1$ is a large positive hyperparameter to substitute $-\log (1-h'_\psi(u,i))$.
% subsubsection find_negative (end)

\textbf{Denoising Negative}. % (fold)
In this sub-task, we only focus on denoising noisy negative examples in the sampled missing interactions, which means that we will regard every positive examples as a clean example.
% , as shown in Figure \ref{fig:FP}.  
That is to say, given $r_{ui} = 0$ we will always have $\tilde{r}_{ui}=0$ (i.e., $h_\phi(u,i)=0$). Thus in this sub-task, only model $h'_\psi$ will be trained. The term $E[\log P(\tilde{\textbf{R}}|\textbf{R})]$ is expanded as
\begin{align}
\label{eq:likelihood-dfn}
  &E[\log P(\tilde{\textbf{R}}|\textbf{R})]=\hspace{-0.3cm}\sum_{(u,i)|\tilde{r}_{ui}=0}\hspace{-0.3cm}
   \log(1 - h'_\psi(u,i))\cdot f_{\theta}(u,i) \nonumber \\
 &+\hspace{-0.3cm}\sum_{(u,i)|\tilde{r}_{ui}=1}\hspace{-0.3cm}
    \log h'_\psi(u,i) \cdot f_{\theta}(u,i) -C_2 \cdot (1-f_\theta(u,i)),
 \end{align}
where $C_2$ is a large positive hyperparameter to replace $-\log(h_\phi(u,i))$.
% subsubsection find_positive (end)

In the training procedure of DeCA and DeCA(p), we will expand $E[\log P(\tilde{\textbf{R}}|\textbf{R})]$ as Eq.(\ref{eq:likelihood-dfp}) and Eq.(\ref{eq:likelihood-dfn}) iteratively to denoise both noisy positive examples and noisy negative examples. \wy{The detailed pseudo code is as follows:}


\begin{minipage}{0.46\textwidth}
 \begin{algorithm}[H]
    \small
  % \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \KwIn{Corrupted data $\tilde{\textbf{R}}$, learning rate $\beta$, epochs $T$, hyper-parameter $\alpha, C_1, C_2$, regularization weight $\lambda$, target recommender $f$, auxiliary model $g$, $h$, $h'$}
  \KwOut{Parameters $\theta, \mu, \phi, \psi$ for $f,g,h,h'$, correspondingly}
  Initialize all parameters\;
  $count$ $\leftarrow$ 0\; 
  \While{Not early stop and $epoch < T$}{
    Draw a minibatch of $(u,i_+)$ from $\{(u,i)| \tilde{r}_{ui} = 1\}$\;
    Draw  $(u,i_-)$ from $\{(u,i)| \tilde{r}_{ui} = 0\}$\ for each $(u,i_+)$\;
    % Sample one negative item for each user in the minibatch and constitute $k$ minibatches of $(u,i_-)$ from $\{(u,i)| \tilde{r}_{ui} = 0\}$\;
    \uIf{$count \% 2 == 0$}{
      Compute $\mathcal{L}_{DeCA}$ according to Eq.(\ref{DPI-loss}) and Eq.(\ref{eq:likelihood-dfp})\;
    }
    \uElse{
      Compute $\mathcal{L}_{DeCA}$ according to Eq.(\ref{DPI-loss}) and Eq.(\ref{eq:likelihood-dfn})\;
    }
    Add regularization term: $\mathcal{L}_{DeCA} \leftarrow \mathcal{L}_{DeCA} + \lambda||\theta||^2$\;
    \For{each parameter $\Theta$ in $\{\theta, \mu, \phi, \psi\}$}{
      Compute $\partial \mathcal{L}_{DeCA} / \partial \Theta$ by back-propagation\;
      $\Theta \leftarrow \Theta - \beta \partial \mathcal{L}_{DeCA}/\partial \Theta$
    }
    $count$ $\leftarrow$ $count+1$\; 
  }
  \caption{Learning algorithm for DeCA}
  \label{alg:DPI}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
\scriptsize
  \KwIn{Corrupted data $\tilde{\textbf{R}}$, learning rate $\beta$, epochs $T$, hyper-parameter $\alpha, C_1, C_2$, regularization weight $\lambda$, target recommender $f$, auxiliary model $h$, $h'$}
  \KwOut{Parameters $\theta, \phi, \psi$ for $f,h,h'$, correspondingly}
  Set random seed to $s_1$, initialize another copy of $\theta$ as $\theta'$\;
  \While{Not early stop and $epoch < T$}{
    Draw a minibatch of $(u,i_+)$ from $\{(u,i)| \tilde{r}_{ui} = 1\}$\;
    Draw  $(u,i_-)$ from $\{(u,i)| \tilde{r}_{ui} = 0\}$\ for each $(u,i_+)$\;
    Compute binary cross-entropy 
    $\mathcal{L}_{BCE}$ on $(u,i_+)$ and $(u,i_-)$ with $f_{\theta'}$\;
    Add regularization: $\mathcal{L}_{BCE} \leftarrow \mathcal{L}_{BCE} + \lambda||\theta'||^2$\;
    Compute $\partial \mathcal{L}_{BCE}/\partial \theta'$ by back-propagation\;
    $\theta' \leftarrow \theta' - \beta \partial \mathcal{L}/\partial \theta'$\;
  }
  Freeze $\theta'$, set random seed to $s_2$ and initialize $\theta, \phi, \psi$\; 
  $count$ $\leftarrow$ 0\; 
  \While{Not early stop and $epoch < T$}{
    Draw $(u,i_+)$ and $(u,i_-)$ similarly with line3-4\;
    \uIf{$count \% 2 == 0$}{
      Compute $\mathcal{L}_{DeCA(p)}$ according to Eq.(\ref{DVAE-loss}) and Eq.(\ref{eq:likelihood-dfp})\;
    }
    \uElse{
      Compute $\mathcal{L}_{DeCA(p)}$ according to Eq.(\ref{DVAE-loss}) and Eq.(\ref{eq:likelihood-dfn})\;
    }
    Add regularization term: $\mathcal{L}_{DeCA(p)} \leftarrow \mathcal{L}_{DeCA(p)} + \lambda||\theta||^2$\;
    \For{each parameter $\Theta$ in $\{\theta, \phi, \psi\}$}{
      Compute $\partial \mathcal{L}_{DeCA(p)} / \partial \Theta$ by back-propagation\;
      $\Theta \leftarrow \Theta - \beta \partial \mathcal{L}_{DeCA(p)}/\partial \Theta$\;
    }
    $count$ $\leftarrow$ $count+1$\; 
  }
  \caption{Learning algorithm for DeCA(p)}
  \label{alg:DVAE}
\end{algorithm}
\end{minipage}

% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c}
%         \toprule
%          \begin{algorithm}
%     \small
%   % \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%   \KwIn{Corrupted data $\tilde{\textbf{R}}$, learning rate $\beta$, epochs $T$, hyper-parameter $\alpha, C_1, C_2$, regularization weight $\lambda$, target recommender $f$, auxiliary model $g$, $h$, $h'$}
%   \KwOut{Parameters $\theta, \mu, \phi, \psi$ for $f,g,h,h'$, correspondingly}
%   Initialize all parameters\;
%   $count$ $\leftarrow$ 0\; 
%   \While{Not early stop and $epoch < T$}{
%     Draw a minibatch of $(u,i_+)$ from $\{(u,i)| \tilde{r}_{ui} = 1\}$\;
%     Draw  $(u,i_-)$ from $\{(u,i)| \tilde{r}_{ui} = 0\}$\ for each $(u,i_+)$\;
%     % Sample one negative item for each user in the minibatch and constitute $k$ minibatches of $(u,i_-)$ from $\{(u,i)| \tilde{r}_{ui} = 0\}$\;
%     \uIf{$count \% 2 == 0$}{
%       Compute $\mathcal{L}_{DeCA}$ according to Eq.(\ref{DPI-loss}) and Eq.(\ref{eq:likelihood-dfp})\;
%     }
%     \uElse{
%       Compute $\mathcal{L}_{DeCA}$ according to Eq.(\ref{DPI-loss}) and Eq.(\ref{eq:likelihood-dfn})\;
%     }
%     Add regularization term: $\mathcal{L}_{DeCA} \leftarrow \mathcal{L}_{DeCA} + \lambda||\theta||^2$\;
%     \For{each parameter $\Theta$ in $\{\theta, \mu, \phi, \psi\}$}{
%       Compute $\partial \mathcal{L}_{DeCA} / \partial \Theta$ by back-propagation\;
%       $\Theta \leftarrow \Theta - \beta \partial \mathcal{L}_{DeCA}/\partial \Theta$
%     }
%     $count$ $\leftarrow$ $count+1$\; 
%   }
%   \caption{Learning algorithm for DeCA}
%   \label{alg:DPI}
% \end{algorithm} & 
% \begin{algorithm}
% \footnotesize
%   \KwIn{Corrupted data $\tilde{\textbf{R}}$, learning rate $\beta$, epochs $T$, hyper-parameter $\alpha, C_1, C_2$, regularization weight $\lambda$, target recommender $f$, auxiliary model $h$, $h'$}
%   \KwOut{Parameters $\theta, \phi, \psi$ for $f,h,h'$, correspondingly}
%   Set random seed to $s_1$, initialize another copy of $\theta$ as $\theta'$\;
%   \While{Not early stop and $epoch < T$}{
%     Draw a minibatch of $(u,i_+)$ from $\{(u,i)| \tilde{r}_{ui} = 1\}$\;
%     Draw  $(u,i_-)$ from $\{(u,i)| \tilde{r}_{ui} = 0\}$\ for each $(u,i_+)$\;
%     Compute binary cross-entropy 
%     $\mathcal{L}_{BCE}$ on $(u,i_+)$ and $(u,i_-)$ with $f_{\theta'}$\;
%     Add regularization: $\mathcal{L}_{BCE} \leftarrow \mathcal{L}_{BCE} + \lambda||\theta'||^2$\;
%     Compute $\partial \mathcal{L}_{BCE}/\partial \theta'$ by back-propagation\;
%     $\theta' \leftarrow \theta' - \beta \partial \mathcal{L}/\partial \theta'$\;
%   }
%   Freeze $\theta'$, set random seed to $s_2$ and initialize $\theta, \phi, \psi$\; 
%   $count$ $\leftarrow$ 0\; 
%   \While{Not early stop and $epoch < T$}{
%     Draw $(u,i_+)$ and $(u,i_-)$ similarly with line3-4\;
%     \uIf{$count \% 2 == 0$}{
%       Compute $\mathcal{L}_{DeCA(p)}$ according to Eq.(\ref{DVAE-loss}) and Eq.(\ref{eq:likelihood-dfp})\;
%     }
%     \uElse{
%       Compute $\mathcal{L}_{DeCA(p)}$ according to Eq.(\ref{DVAE-loss}) and Eq.(\ref{eq:likelihood-dfn})\;
%     }
%     Add regularization term: $\mathcal{L}_{DeCA(p)} \leftarrow \mathcal{L}_{DeCA(p)} + \lambda||\theta||^2$\;
%     \For{each parameter $\Theta$ in $\{\theta, \phi, \psi\}$}{
%       Compute $\partial \mathcal{L}_{DeCA(p)} / \partial \Theta$ by back-propagation\;
%       $\Theta \leftarrow \Theta - \beta \partial \mathcal{L}_{DeCA(p)}/\partial \Theta$\;
%     }
%     $count$ $\leftarrow$ $count+1$\; 
%   }
%   \caption{Learning algorithm for DeCA(p)}
%   \label{alg:DVAE}
% \end{algorithm}
% \\
%          \bottomrule
%     \end{tabular}
% \end{table}






% subsection denoising_with_variational_inference (end)


\subsection{Extension to Multi-class Scenario}
% \section{Method}
In this section, we extend the proposed DeCA methods from the binary scenario to the multi-class scenario.

\subsubsection{Notations and Problem Formulation}
We use $\tilde{\textbf{y}} \in \mathbb{R}^{N}$ or $\{\tilde{y}_i\}_{i=1}^N$ to denote the noisy labels, while using $\textbf{y} \in \mathbb{R}^{N}$ or $\{y_i\}_{i=1}^N$ to denote underlying true labels. We focus on multi-class classification problems here, which means $\tilde{y}_i, y_i \in \{1, \cdots, C\}$, where $C$ refers to the total number of classes. Besides, $\textbf{x}$ or $\{x_i\}_{i=1}^N$ denote the features (e.g., the input images). 
% We believe there is some correlation between $\tilde{\textbf{y}}$ and $\textbf{y}$ given $x$. 
% \wy{The correlations between $\textbf{x}$, $\textbf{y}$ and $\tilde{\textbf{y}}$ are shown in figure \ref{fig:variable_correlations}.}
We assume $\tilde{\textbf{y}}$ and $\textbf{y}$ are drawn from multinomial distribution. 
% To summarize, we have the following two assumptions.
The assumptions in this papar are summarized as follows:
% \begin{wrapfigure}{r}{0.2\textwidth}
% % \vspace{-12pt}
% \centering
% \includegraphics[width=\linewidth]{figures/PVD_causal_graph.pdf}
% \caption{Correlations between $\textbf{x}$, $\textbf{y}$ and $\tilde{\textbf{y}}$. }
% \vspace{-0.3cm}
% \label{fig:variable_correlations}
% \end{wrapfigure}
\begin{assumption}\label{assumption_1}
True label $y_i$ is drawn from a multinomial distribution conditioned on $x_i$ and is not dependent on $\tilde{y}_i$:
\begin{equation}\label{encoder}
% \displaywidth=\parshapelength\numexpr\prevgraf+2\relax
    y_i|(x_i, \tilde{y}_i) \sim Mult(C, \eta_i) \approx Mult(C, f_\theta(x_i, \tilde{y}_i))
\end{equation}
where $\eta_i \in \mathbb{R}^{C}$ describes the probability distribution of $i$-th example over all $C$ classes and is approximated by $f_\theta(x_i, \tilde{y_i})$. $\theta$ denote the parameter of function $f$. $Multi(C, \eta_i)$ refers to the multinomial distribution with the probabilities $\eta_i$. 
% We argue that we can incorporate the effects of noisy label $\tilde{y}_i$ as the condition into $f_\theta$. 
\end{assumption}

Based on Assumption \ref{assumption_1}, during implementation we will only input $x_i$ into the model $f_\theta$. We argue that the true labels $y_i$ mainly depend on the features $x_i$ rather than the noisy label $y_i$, \emph{i.e.}, the information from $\tilde{\textbf{y}}$ is trivial.
%(2) the model $f_\theta$ should incorporate the trivial information from $\tilde{\textbf{y}}$ into the parameters. Thus in the following, we will use $f_\theta(x_i)$ to replace $f_\theta(x_i, \tilde{y}_i)$ in Eq.(\ref{encoder}).

\begin{assumption}
Given true label $y_i$ and the feature $x_i$, the observed noisy label $\tilde{y}_i$ is also drawn from a multinomial distribution:
\begin{equation}\label{decoder}
% \displaywidth=\parshapelength\numexpr\prevgraf+2\relax
    \tilde{y}_i | x_i, y_i \sim Mult(C, h_\phi(x_i, y_i)) 
\end{equation}
where $h_\phi$ is the model representing the mapping from $(x_i, y_i)$ to $\tilde{y}_i$, and $\phi$ is the parameters of the model. With $h_\phi$ we are able to describe the correlation between $x_i, y_i$ and $\tilde{y}_i$. 
\end{assumption}

Now the problem of this work is to infer the distribution of true labels $\textbf{y}$ given the noisy observed labels $\tilde{\textbf{y}}$ and the features $\textbf{x}$. Note that when dealing with binary classification problems in the recommendation systems, the multinomial distribution will degenerate to binomial distribution.

\subsubsection{Label Denoising with Cross-model Agreement}
In order to infer the true distribution of $\textbf{y}$, we first denote the distribution of $\textbf{y}$ given observed labels $\tilde{\textbf{y}}$ and the features $\textbf{x}$ as $Q_f(\textbf{y}|\tilde{\textbf{y}}, \textbf{x})$, parameterized by $f_\theta$. In the following part, we will omit $\textbf{x}$ as the condition, since all the probabilities mentioned below are conditioned on $\textbf{x}$. We try to minimize the KL-divergence between $Q_f(\textbf{y}|\tilde{\textbf{y}})$ and the true conditional distribution $P(\textbf{y}|\tilde{\textbf{y}})$: 
\begin{equation}\label{KL-divergence}
 \min  \mathcal{D}_{KL}[Q_f(\textbf{y}|\tilde{\textbf{y}}) || P(\textbf{y}|\tilde{\textbf{y}})]
\end{equation}
However, the probability $P(\textbf{y} | \tilde{\textbf{y}})$ is intractable to calculate, thus we use bayesian equation to expand $P(\textbf{y}|\tilde{\textbf{y}})$ to $P(\textbf{y}) P(\tilde{\textbf{y}}|\textbf{y}) / P(\tilde{\textbf{y}}) $ and then substitute it back into Eq.(\ref{KL-divergence}), yielding:
\begin{align}\label{expansion}
\mathcal{D}_{KL}[Q_f(\textbf{y}|\tilde{\textbf{y}}) & ||  P(\textbf{y}|\tilde{\textbf{y}})] = E_{\textbf{y}\sim Q_f}[Q_f(\textbf{y}|\tilde{\textbf{y}}) - P(\textbf{y}|\tilde{\textbf{y}})] \nonumber \\
&= E_{\textbf{y}\sim Q_f}[\log Q_f(\textbf{y}|\tilde{\textbf{y}}) - \log P(\textbf{y}) \frac{P(\tilde{\textbf{y}}|\textbf{y})}{P(\tilde{\textbf{y}})}] \nonumber \\
&= E_{\textbf{y}\sim Q_f}[\log Q_f(\textbf{y}|\tilde{\textbf{y}}) - \log P(\textbf{y}) - \log P(\tilde{\textbf{y}}|\textbf{y}) + \log P(\tilde{\textbf{y}})] \nonumber \\
&= \mathcal{D}_{KL} [Q_f(\textbf{y}|\tilde{\textbf{y}})||P(\textbf{y})] - \log P(\tilde{y}) + E_{{\textbf{y}\sim Q_f}}[\log P(\tilde{\textbf{y}} | \textbf{y})]
\end{align}
Then we rearrange the terms in Eq.(\ref{expansion}), and obtain:
\begin{equation}\label{variational_lower_bound}
    \log P(\tilde{\textbf{y}}) - \mathcal{D}_{KL}[Q_f(\textbf{y}|\tilde{\textbf{y}}) ||  P(\textbf{y}|\tilde{\textbf{y}})] = E_{{\textbf{y}\sim Q_f}}[\log P(\tilde{\textbf{y}} | \textbf{y})] - \mathcal{D}_{KL} [Q_f(\textbf{y}|\tilde{\textbf{y}})||P(\textbf{y})]
\end{equation}
% Thus it has become the objective in the variational autoencoder. 
In Eq.(\ref{variational_lower_bound}), $Q_f(\textbf{y}|\tilde{\textbf{y}})$ is our target model denoted in Eq.(\ref{encoder}), while $P(\tilde{\textbf{y}}|\textbf{y})$ has been defined in Eq.(\ref{decoder}). Thus we can expand the right side of Eq.(\ref{expansion}) analytically with defining $P(\textbf{y})$ as the prior distribution.
Thus the denoising objective function can be formulated as:
% \begin{equation}\label{loss}
%     \mathcal{L} = - E_{{\textbf{y}\sim Q_f}}[\log P(\tilde{\textbf{y}} | \textbf{y})] + \mathcal{D}_{KL} [Q_f(\textbf{y}|\tilde{\textbf{y}})||P(\textbf{y})]
% \end{equation}
\begin{equation}\label{loss}
    \mathcal{L} = - E_{{\textbf{y}\sim Q_f}}[\log P(\tilde{\textbf{y}} | \textbf{y})] + \mathcal{D}_{KL} [Q_f(\textbf{y}|\tilde{\textbf{y}})||P(\textbf{y})]
\end{equation}

More precisely, we can give the detailed formulation of the term $E_{\textbf{y}\sim Q_f}[\log P(\tilde{\textbf{y}}|\textbf{y})]$ in $\mathcal{L}$ as:
\begin{align}\label{expansion_of_expectation}
    E_{{\textbf{y}\sim Q_f}}[\log P(\tilde{\textbf{y}} | \textbf{y})] = \sum_i \sum_{c\in \mathcal{C}} \log P(\tilde{y}_i|y_i = c) * P(y_i = c)
\end{align}
Then the KL divergence term $[Q_f(\textbf{y}|\tilde{\textbf{y}})||P(\textbf{y})]$ can be calculated as:
\begin{equation*}
    \mathcal{D}_{KL} [Q_f(\textbf{y}|\tilde{\textbf{y}})||P(\textbf{y})] = f_\theta \cdot \log \frac{f_\theta}{f_\theta'} + (1 - f_\theta) \cdot \log \frac{1 - f_\theta}{1 - f_\theta'}
\end{equation*}
where $f_\theta'$ denote the fixed prior distribution from a pretrained model, which share the same structure as $f_\theta$ and is trained on the noisy dataset. In other words, we extend the pre-trained DeCA(p) for the multi-class scenario.

% \wy{ This setting is motivated by the observation in Figure \ref{fig:Analysis_on_memorizing_noisy_samples_mnist}, which shows that the same model structure trained with different random seeds tends to have more consistent predictions on the clean examples than the noisy examples.In Eq.(\ref{loss}), the first term is the probability of the observation, while the second term is the differences between $f_\theta$ (modeling $Q_f(\textbf{y}|\tilde{\textbf{y}})$) and $f_{\theta'}$ (modeling $P(\textbf{y})$), which should be minimized since the predictions between two models should be consistent on the true labels $\textbf{y}$.}

\subsubsection{Training Routine}
We can see there is a expectation term in Eq.(\ref{loss}): $E_{{\textbf{y}\sim Q_f}}[\log P(\tilde{\textbf{y}} | \textbf{y})]$. A naive solution to optimize $E_{{\textbf{y}\sim Q_f}}[\log P(\tilde{\textbf{y}} | \textbf{y})]$ could be performing calculation as shown in Eq.(\ref{expansion_of_expectation}). However, In our implementaion, it won't yield satisfactory results. The reason is that computing $E_{{\textbf{y}\sim Q_f}}[\log P(\tilde{\textbf{y}} | \textbf{y})]$ requires computing $P(\tilde{\textbf{y}} | \textbf{y})$ (or $h_\phi$ in Eq.(\ref{decoder})) first. 
However, in the early stage of training, the true labels $\textbf{y}$ is hardly inferred by the under-trained model $f_\theta$, and the model $h_\phi$ itself is also corrupted. Then the objective Eq.(\ref{loss}) will fail to refine the model $f_\theta$ or $h_\phi$. Instead, they would stuck on  local minimum where the loss is small but $f_\theta$ and $h_\phi$ are all meaningless.
% The input of this model is $\textbf{x}$ and one of the guessed $|\mathcal{C}|$ classes.
% Each class as the input could affect the results. 
% Thus there are potentially 10 paths in this model, which although are not totally independent. 
% If we directly calculate $E_{{\textbf{y}\sim Q_f}}[\log P(\tilde{\textbf{y}} | \textbf{y})]$ and optimize it in an end-to-end fashion, these $|\mathcal{C}|$ potential paths could interfere with each other and the model could reach a local minimum which is far away from global minimum. 
To handle this issue, we design a specific training routine. 
For the model $h_\phi$ in Eq.(\ref{decoder}), the input $y_i$ has $|\mathcal{C}|$ possible values. We will force the model to attend to one value in each timestep.

\noindent At timestep $T$, let $k = T$ mod $|\mathcal{C}|$. In this step, $\forall c \in \{1,\cdots,\mathcal{C}\}$ we set the probability $P(\tilde{y}_i|y_i)$ as: 

\begin{equation}\label{training_routine_set_conditional_probability}
    P(\tilde{y}_i = c|y_i = c) = \left\{\begin{array}{ll}
        1, & c\neq k \\
        h_\phi(x_i, y_i), & c=k \\
    \end{array}\right.
\end{equation}

\noindent Then Eq.(\ref{expansion_of_expectation}) becomes:

\begin{align}
E[\log P(\tilde{\textbf{R}}|\textbf{R})] &= \sum_{i|\tilde{y}_i=k} \sum_{c\in \mathcal{C} \& c\neq k} -C_1 * P(y_i=c) + \log P(\tilde{y}_i=k|y_i=k) * P(y_i=k) \nonumber \\
& + \sum_{i|\tilde{y}_i\neq k}  \sum_{c \in \mathcal{C} \& c \neq k, c\neq \tilde{y}} -C_2*P(y_i=c) + \log(P(\tilde{y}_i|y_i=k)) P(y_i = k)  \nonumber \\
& = \sum_{i|\tilde{y}_i=k} - C_1 * (1-P(\hat{y_i} = k)) + \log P(\tilde{y}_i=k|y_i=k) * P(y_i=k) \nonumber \\
& + \sum_{i|\tilde{y}_i\neq k}  -C_2 * (1 - P(y_i = k) - P(y_i = \tilde{y}_i)) + \log(P(\tilde{y}_i|y_i=k)) P(y_i = k)  \label{training_objective_1}
\end{align}
% \begin{align}\label{training_objective_1}
% E[\log & P(\tilde{\textbf{R}}|\textbf{R})] = \left\{\begin{array}{l}
% 		\displaystyle \sum_{i|\tilde{y}_i=k} \sum_{c\in \mathcal{C} \& c\neq k} -C_1 * P(y_i=c) + \log P(\tilde{y}_i=k|y_i=k) * P(y_i=k) \\
% 		\displaystyle \sum_{i|\tilde{y}_i\neq k}  \sum_{c \in \mathcal{C} \& c \neq k, c\neq \tilde{y}} -C_2*P(y_i=c) + \log(P(\tilde{y}_i|y_i=k)) P(y_i = k) 
% 	\end{array}\right. \nonumber \\
% 	& = \left\{\begin{array}{l}
% 		\displaystyle \sum_{i|\tilde{y}_i=k} - C_1 * (1-P(\hat{y_i} = k)) + \log P(\tilde{y}_i=k|y_i=k) * P(y_i=k) \\
% 		\displaystyle \sum_{i|\tilde{y}_i\neq k}  -C_2 * (1 - P(y_i = k) - P(y_i = \tilde{y}_i)) + \log(P(\tilde{y}_i|y_i=k)) P(y_i = k) 
% 	\end{array}\right.
% \end{align}
where $C_1$ is the large positive hyper-parameter used to substitute the $-\log (P(\tilde{y}_i = k | y_i = c)), \forall c \in \mathcal{C} \backslash \{k\}$, and $C_2$ is another large positive hyper-parameter representing $-\log (P(\tilde{y}_i| y_i = c)), \forall c \in \mathcal{C} \backslash \{k, \tilde{y}_i\}$. Intuitively, we constrain all the correlations between $c\neq k$, $y$ and $\tilde{y}$ but leave the function lying between $\tilde{y}$ and $k$ unconstrained, denoted by $P(\tilde{y}_i|y_i=k)$. Thus the objective of current step is to learn the part that is only correlated with $y_i = k$ in $h_\phi$. 

After certain epochs, when the probability distributions parameterized by $h_\phi$ have converged, we can remove $C_1$ and $C_2$ and change Eq.(\ref{training_routine_set_conditional_probability}) to:
\begin{equation}
     P(\tilde{y}_i = c|y_i = c) = \left\{\begin{array}{ll}
        SG(h_\phi(x_i, y_i)), & c\neq k \\
        h_\phi(x_i, y_i), & c=k \\
    \end{array}\right.
\end{equation}
where $SG$ imeans stop-gradient. Then the objective in Eq.(\ref{training_objective_1}) will be:
\begin{align*}
    E[\log & P(\tilde{\textbf{R}}|\textbf{R})] = \left\{\begin{array}{l}
		\displaystyle \sum_{i|\tilde{y}_i=k} \sum_{c\in \mathcal{C} \& c\neq k} SG(\log P(k|y_i=c)) * P(y_i=c) + \log P(k|y_i=k) * P(y_i=k) \\
		\displaystyle \sum_{i|\tilde{y}_i\neq k} \sum_{c \in \mathcal{C} \& c \neq k, c\neq \tilde{y}} SG(\log P(\tilde{y}_i|y_i=c)) *P(y_i=c) + \log(P(\tilde{y}_i|y_i=k)) P(y_i = k)
	\end{array}\right.
\end{align*}




\subsection{Discussion}

In this subsection, we provide a brief discussion to illustrate the relationship between our methods and other related methods.  
\subsubsection{Relationship with Variational Auto-Encoder}
We can see that Eq.(\ref{VAE_lower_bound}) is exactly the objective function of a variational auto-encoder (VAE) \cite{doersch2016vaetutorial}.
Specifically, the real user preference $\textbf{R}$ is the latent variable. $P_f(\textbf{R}|\tilde{\textbf{R}})$ which is parameterized by our target model $f_\theta$ maps the corrupted data $\tilde{\textbf{R}}$ to the latent variables $\textbf{R}$ and thus can be seen as the encoder. The likelihood $P(\tilde{\textbf{R}}|\textbf{R})$ describes the distribution of corrupted data $\tilde{\textbf{R}}$ given the real user preference $\textbf{R}$ and acts as the decoder. Finally, $P(\mathbf{R})$ is the fixed prior distribution. However, we claim that the proposed DeCA(p) is substantially different from VAE. For example, DeCA(p) does not utilize the re-parameterization of VAE. VAE is just an interpretation of DeCA(p). Besides, although there are some methods utilizing VAE for recommendation ~\cite{DBLP:conf/www/LiangKHJ18,DBLP:conf/wsdm/ShenbinATMN20}, few of them are designed for recommendation denoising. Finally, existing VAE-based recommendation methods are actually recommendation models while the proposed DeCA(p) acts a \emph{model-agnostic training framework} which is then instantiated with all kinds of downstream models. They serve on different levels.  

% \subsubsection{Analysis of the Convergence}
% During training, if the parameters $C_1$ and $C_2$ are large enough, the process will act similarly to the normal training, since (1) the gradients from the fixed part will dominate the update of the model when $C_1$ and $C_2$ are large. (2) With large $C_1$ and $C_2$, we will demonstrate that the objective has the same target as cross-entropy loss as follows. 

% If we simply replace $-\log(1-h'_\psi(u, i))$ and $-\log(1-h_\phi(u, i))$ with $C_1$ and $C_2$ in the term $E[\log P(\tilde{\textbf{R}}|\textbf{R})]$, we could obtain the following expansion: 
% \begin{equation}\label{eq:expansion}
%     E[\log P(\tilde{\textbf{R}}|\textbf{R})] = - \sum_{(u,i)|\tilde{r}_{ui} = 0} C_1 \cdot f_\theta(u,i) - \sum_{(u,i)|\tilde{r}_{ui} = 1} C_2 \cdot (1 - f_\theta(u,i))
% \end{equation}
% Thus maximizing Eq.(\ref{eq:expansion}) will optimize $f_\theta(u,i)$ to fit the observational data. The loss for the dataset is similar to cross-entropy loss, and it will converge. 

\subsubsection{Analysis of the Run Time Complexity}
For DeCA, the main additional complexity comes from the forward and backward of the auxiliary model. DeCA also incorporates information from different models. However, compared with ensemble methods, DeCA only uses the target model for inference while ensemble methods need the forward pass of each model. As a result, DeCA is more efficient than ensemble methods in the inference stage.  


% $g_\mu$. However, since MF is the simplest model, the time complexity will be much smaller than twice the complexity of normal training. 

% For DeCA(p), the total time complexity will be almost exactly twice of normal training, since  the complexity of the second time is almost the same as the first time, i.e., normal training.






















